Rank Vertex Cover as a Natural Problem for Algebraic Compression

The question of the existence of a polynomial kernelization of the Vertex Cover Above LP problem has been a longstanding, notorious open problem in Parameterized Complexity. Five years ago, the breakthrough work by Kratsch and Wahlstrom on representative sets has finally answered this question in the affirmative [FOCS 2012]. In this paper, we present an alternative, algebraic compression of the Vertex Cover Above LP problem into the Rank Vertex Cover problem. Here, the input consists of a graph G, a parameter k, and a bijection between V (G) and the set of columns of a representation of a matriod M, and the objective is to find a vertex cover whose rank is upper bounded by k.

==> TitlePage.tex <==
\conferenceinfo{ISSAC}{University of Kaiserslautern, Germany, 2017}

\title{Rank Vertex Cover as a Natural Problem for Algebraic Compression\titlenote{The research leading to these results has received funding from the European Research Council under the European Union's Seventh Framework Programme (FP7/2007-2013) / ERC grant agreement no. 306992.}}

\numberofauthors{4}

\author{
% You can go ahead and credit any number of authors here,
% e.g. one 'row of three' or two rows (consisting of one row of three
% and a second row of one, two or three).
%
% The command \alignauthor (no curly braces needed) should
% precede each author name, affiliation/snail-mail address and
% e-mail address. Additionally, tag each line of
% affiliation/address with \affaddr, and tag the
% e-mail address with \email.
%
% 1st. author
\alignauthor
S. M. Meesum\\
       \affaddr{The Institute of Mathematical Sciences, HBNI, Chennai, India}\\
       \email{meesum@imsc.res.in}
% 2nd. author
\alignauthor
Saket Saurabh\\
       \affaddr{The Institute of Mathematical Sciences, HBNI, Chennai, India}\\
       \affaddr{University of Bergen, Norway}\\
       \email{saket@imsc.res.in}
% 3rd. author
\alignauthor
Fahad Panolan\\
       \affaddr{University of Bergen, Norway}\\
       \email{fahad.panolan@ii.uib.no}
\and  % use '\and' if you need 'another row' of author names
% 4th. author
\alignauthor Meirav Zehavi\\
       \affaddr{University of Bergen, Norway}\\
       \email{meirav.zehavi@ii.uib.no}
}

\date{04 Febuary 2017}

\maketitle

\begin{abstract}
%It was Lov\'asz \cite{flats} who introduced the concept of associating a matroid with a graph and then using the operations of contraction and deletion in the graph as well as the matroid to study the properties of $\tau$-critical graphs. 
%We make these techniques constructive and use them for compressing  {\sc Above Guarantee Vertex Cover} instances to an instance of \rvc problem, where the guarantee is over the maximum matching value $\lp{}$. In particular, given a graph $H$, a parameter $k$ and a probability $\varepsilon$, we compress the instance $(H,\lp{H}+k)$ of {\sc Above Guarantee Vertex Cover} to an instance $(H',M',k')$ of \rvc in polynomial time with one sided failure probability of at most $\varepsilon$. The instance $(H',M',k')$ has a bit-length of $\OO^*(k^6+k^3\log(1/\varepsilon))$; where $H'$ is a graph, $M'$ is a matrix representing a matroid and $k'$ is a parameter of the order $\OO(k\log k)$.
The question of the existence of a polynomial kernelization of the {\sc Vertex Cover 
Above LP} problem has been a longstanding, notorious open problem in Parameterized Complexity. Five years ago, the breakthrough work by Kratsch and Wahlstr$\ddot{\mathrm{o}}$m on representative sets has finally answered this question in the affirmative [FOCS 2012]. In this paper, we present an alternative, {\em algebraic compression} of the {\sc Vertex Cover 
Above LP} problem into the {\sc Rank Vertex Cover} problem. Here, the input consists of a graph $G$, a parameter $k$, and a bijection between $V(G)$ and the set of columns of a representation of a matriod $M$, and the objective is to find a vertex cover whose rank is upper bounded by $k$.
\end{abstract}

% A category with the (minimum) three required fields
\category{G.2.2}{Graph Theory}{Graph Algorithms}
\category{I.1.2}{Algorithms}{Algebraic Algorithms}
\category{I.1.2}{Algorithms}{Analysis of Algorithms}

%\terms{Theory}

\keywords{Parameterized Complexity, Vertex Cover, Matroid Theory, Polynomial Compression}

